Trimming the Independent Fat: Sufficient Statistics, Mutual Information, and Predictability from Effective Channel States

One of the most fundamental questions one can ask about a pair of random variables X and Y is the value of their mutual information. Unfortunately, this task is often stymied by the extremely large dimension of the variables. We might hope to replace each variable by a lower-dimensional representation that preserves the relationship with the other variable. The theoretically ideal implementation is the use of minimal sufficient statistics, where it is well-known that either X or Y can be replaced by their minimal sufficient statistic about the other while preserving the mutual information. While intuitively reasonable, it is not obvious or straightforward that both variables can be replaced simultaneously. We demonstrate that this is in fact possible: the information X's minimal sufficient statistic preserves about Y is exactly the information that Y's minimal sufficient statistic preserves about X. As an important corollary, we consider the case where one variable is a stochastic process' past and the other its future and the present is viewed as a memoryful channel. In this case, the mutual information is the channel transmission rate between the channel's effective states. That is, the past-future mutual information (the excess entropy) is the amount of information about the future that can be predicted using the past. Translating our result about minimal sufficient statistics, this is equivalent to the mutual information between the forward- and reverse-time causal states of computational mechanics. We close by discussing multivariate extensions to this use of minimal sufficient statistics.

==> cmechabbrev.tex <==
% i thought this was provided by mathtools?
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Abbreviations from CMPPSS:

\newcommand{\eM}     {\mbox{$\epsilon$-machine}\xspace}
\newcommand{\eMs}    {\mbox{$\epsilon$-machines}\xspace}
\newcommand{\EM}     {\mbox{$\epsilon$-Machine}\xspace}
\newcommand{\EMs}    {\mbox{$\epsilon$-Machines}\xspace}
\newcommand{\eT}     {\mbox{$\epsilon$-transducer}\xspace}
\newcommand{\eTs}    {\mbox{$\epsilon$-transducers}\xspace}
\newcommand{\ET}     {\mbox{$\epsilon$-Transducer}\xspace}
\newcommand{\ETs}    {\mbox{$\epsilon$-Transducers}\xspace}

% cryptic
\newcommand{\order}[1]{order\protect\nobreakdash-$#1$}
\newcommand{\Order}[1]{Order\protect\nobreakdash-$#1$}
\newcommand{\cryptic}[1]{$#1$\protect\nobreakdash-cryptic}
\newcommand{\Cryptic}[1]{$#1$\protect\nobreakdash-Cryptic}
\newcommand{\crypticity}[1]{$#1$\protect\nobreakdash-crypticity}
\newcommand{\Crypticity}[1]{$#1$\protect\nobreakdash-Crypticity}

% Processes and sequences

\newcommand{\Process}{\mathcal{P}}

\newcommand{\ProbMach}{\Prob_{\mathrm{M}}}
\newcommand{\Lmax}   { {L_{\mathrm{max}}}}
\newcommand{\MeasAlphabet}      {\mathcal{A}}
% Original symbol
%\newcommand{\MeasSymbol}   { {S} }
%\newcommand{\meassymbol}   { {s} }
% New symbol
\newcommand{\MeasSymbol}   { {X} }
\newcommand{\meassymbol}   { {x} }
\newcommand{\BiInfinity}        { \smash{\overleftrightarrow {\MeasSymbol}} }
\newcommand{\biinfinity}        { \smash{\overleftrightarrow {\meassymbol}} }
\newcommand{\Past}      { \smash{\overleftarrow {\MeasSymbol}} }
\newcommand{\past}      { \smash{\overleftarrow {\meassymbol}} }
\newcommand{\pastprime} { {\past}^{\prime}}
\newcommand{\Future}    { \smash{\overrightarrow{\MeasSymbol}} }
\newcommand{\future}    { \smash{\overrightarrow{\meassymbol}} }
\newcommand{\futureprime}       { \smash{\future^{\prime}} }
\newcommand{\PastPrime}     { \smash{\Past^{\prime}} }
\newcommand{\FuturePrime}       { \smash{\overrightarrow{\meassymbol}^\prime} }
\newcommand{\PastDblPrime}      { \smash{\overleftarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\FutureDblPrime}{ \smash{\overrightarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\pastL}     { \smash{\overleftarrow {\meassymbol}{}^L} }
\newcommand{\PastL}     { \smash{\overleftarrow {\MeasSymbol}{}^L} }
\newcommand{\PastLt}      { \smash{\overleftarrow {\MeasSymbol}_t^L} }
\newcommand{\PastLLessOne}{ \smash{\overleftarrow {\MeasSymbol}^{L-1}} }
\newcommand{\futureL}     { \smash{\overrightarrow{\meassymbol}{}^L} }
\newcommand{\FutureL}     { \smash{\overrightarrow{\MeasSymbol}{}^L} }
\newcommand{\FutureLt}    { \smash{\overrightarrow{\MeasSymbol}_t^L} }
\newcommand{\FutureLLessOne}{ \smash{\overrightarrow{\MeasSymbol}^{L-1}} }
\newcommand{\pastLprime}        { \smash{\overleftarrow {\meassymbol}^{L^\prime}} }
\newcommand{\futureLprime}      { \smash{\overrightarrow{\meassymbol}^{L^\prime}} }
\newcommand{\AllPasts}      { \smash{\overleftarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\AllFutures}        { \smash{\overrightarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\FutureSet} { \smash{\overrightarrow{\bf \MeasSymbol}} }

% Causal states and epsilon-machines
\newcommand{\CausalState}       { \mathcal{S} }
\newcommand{\CausalStatePrime}  { {\CausalState}^{\prime}}
\newcommand{\causalstate}       { \sigma }
\newcommand{\CausalStateSet}    { \boldsymbol{\CausalState} }
\newcommand{\AlternateState}    { \mathcal{R} }
\newcommand{\AlternateStatePrime}       { {\cal R}^{\prime} }
\newcommand{\alternatestate}    { \rho }
\newcommand{\alternatestateprime}       { {\rho^{\prime}} }
\newcommand{\AlternateStateSet} { \boldsymbol{\AlternateState} }
\newcommand{\PrescientState}    { \widehat{\AlternateState} }
\newcommand{\prescientstate}    { \widehat{\alternatestate} }
\newcommand{\PrescientStateSet} { \boldsymbol{\PrescientState}}
\newcommand{\CausalEquivalence} { {\sim}_{\epsilon} }
\newcommand{\CausalEquivalenceNot}      { {\not \sim}_{\epsilon}}

\newcommand{\NonCausalEquivalence}      { {\sim}_{\eta} }
\newcommand{\NextObservable}    { {\smash{\overrightarrow {\MeasSymbol}}^1} }
\newcommand{\LastObservable}    { {\smash{\overleftarrow {\MeasSymbol}}^1} }
%\newcommand{\Prob}             { {\rm P}}
\newcommand{\Prob}      {\Pr} % use standard command
\newcommand{\ProbAnd}   { {,\;} }
\newcommand{\LLimit}    { {L \rightarrow \infty}}
\newcommand{\Cmu}               {C_\mu}
\newcommand{\hmu}               {h_\mu}
\newcommand{\EE}                {{\bf E}}
\newcommand{\TI}                {{\bf T}}
\newcommand{\SyncI}        {{\bf S}}
\newcommand{\Measurable}{{\bf \mu}}

% Process Crypticity
\newcommand{\PC}                {\chi}

% Causal Irreversibility
\newcommand{\CI}                {\Xi}
\newcommand{\ReverseMap}        {r}
\newcommand{\ForwardMap}        {f}

% Abbreviations from IB:
% None that aren't already in CMPPSS

% Abbreviations from Extensive Estimation:
\newcommand{\EstCausalState}    {\widehat{\CausalState}}
\newcommand{\estcausalstate}    {\widehat{\causalstate}}
\newcommand{\EstCausalStateSet} {\boldsymbol{\EstCausalState}}
\newcommand{\EstCausalFunc}     {\widehat{\epsilon}}
\newcommand{\EstCmu}            {\widehat{\Cmu}}
\newcommand{\PastLOne}  {{\Past}^{L+1}}
\newcommand{\pastLOne}  {{\past}^{L+1}}

% Abbreviations from $\epsilon$-Transducers:
\newcommand{\InAlphabet}        { \mathcal{A}}
\newcommand{\insymbol}          { a}
\newcommand{\OutAlphabet}       { \mathcal{B}}
\newcommand{\outsymbol}         { b}
\newcommand{\InputSimple}       { X}
\newcommand{\inputsimple}       { x}
\newcommand{\BottleneckVar}     {\tilde{\InputSimple}}
\newcommand{\bottleneckvar}     {\tilde{\inputsimple}}
\newcommand{\InputSpace}        { \mathbf{\InputSimple}}
\newcommand{\InputBi}   { \overleftrightarrow {\InputSimple} }
\newcommand{\inputbi}   { \overleftrightarrow {\inputsimple} }
\newcommand{\InputPast} { \overleftarrow {\InputSimple} }
\newcommand{\inputpast} { \overleftarrow {\inputsimple} }
\newcommand{\InputFuture}       { \overrightarrow {\InputSimple} }
\newcommand{\inputfuture}       { \overrightarrow {\inputsimple} }
\newcommand{\NextInput} { {{\InputFuture}^{1}}}
\newcommand{\NextOutput}        { {\OutputFuture}^{1}}
\newcommand{\OutputSimple}      { Y}
\newcommand{\outputsimple}      { y}
\newcommand{\OutputSpace}       { \mathbf{\OutputSimple}}
\newcommand{\OutputBi}  { \overleftrightarrow{\OutputSimple} }
\newcommand{\outputbi}  { \overleftrightarrow{\outputsimple} }
\newcommand{\OutputPast}        { \overleftarrow{\OutputSimple} }
\newcommand{\outputpast}        { \overleftarrow{\outputsimple} }
\newcommand{\OutputFuture}      { \overrightarrow{\OutputSimple} }
\newcommand{\outputfuture}      { \overrightarrow{\outputsimple} }
\newcommand{\OutputL}   { {\OutputFuture}^L}
\newcommand{\outputL}   { {\outputfuture}^L}
\newcommand{\InputLLessOne}     { {\InputFuture}^{L-1}}
\newcommand{\inputLlessone}     { {\inputufutre}^{L-1}}
\newcommand{\OutputPastLLessOne}        {{\OutputPast}^{L-1}_{-1}}
\newcommand{\outputpastLlessone}        {{\outputpast}^{L-1}}
\newcommand{\OutputPastLessOne} {{\OutputPast}_{-1}}
\newcommand{\outputpastlessone} {{\outputpast}_{-1}}
\newcommand{\OutputPastL}       {{\OutputPast}^{L}}
\newcommand{\OutputLPlusOne}    { {\OutputFuture}^{L+1}}
\newcommand{\outputLplusone}    { {\outputfutre}^{L+1}}
\newcommand{\InputPastL}        {{\InputPast}^{L}}
\newcommand{\inputpastL}        {{\inputpast}^{L}}
\newcommand{\JointPast} {{(\InputPast,\OutputPast)}}
\newcommand{\jointpast} {{(\inputpast,\outputpast)}}
\newcommand{\jointpastone}      {{(\inputpast_1,\outputpast_1)}}
\newcommand{\jointpasttwo}      {{(\inputpast_2,\outputpast_2)}}
\newcommand{\jointpastprime} {{({\inputpast}^{\prime},{\outputpast}^{\prime})}}
\newcommand{\NextJoint} {{(\NextInput,\NextOutput)}}
\newcommand{\nextjoint} {{(\insymbol,\outsymbol)}}
\newcommand{\AllInputPasts}     { { \overleftarrow {\rm \InputSpace}}}
\newcommand{\AllOutputPasts}    { {\overleftarrow {\rm \OutputSpace}}}
\newcommand{\DetCausalState}    { {{\cal S}_D }}
\newcommand{\detcausalstate}    { {{\sigma}_D} }
\newcommand{\DetCausalStateSet} { \boldsymbol{{\CausalState}_D}}
\newcommand{\DetCausalEquivalence}      { {\sim}_{{\epsilon}_{D}}}
\newcommand{\PrescientEquivalence}      { {\sim}_{\widehat{\eta}}}
\newcommand{\FeedbackCausalState}       { \mathcal{F}}
\newcommand{\feedbackcausalstate}       { \phi}
\newcommand{\FeedbackCausalStateSet}    { \mathbf{\FeedbackCausalState}}
\newcommand{\JointCausalState}          { \mathcal{J}}
\newcommand{\JointCausalStateSet}       { \mathbf{\JointCausalState}}
\newcommand{\UtilityFunctional} { {\mathcal{L}}}
\newcommand{\NatureState}       { {\Omega}}
\newcommand{\naturestate}       { {\omega}}
\newcommand{\NatureStateSpace}  { {\mathbf{\NatureState}}}
\newcommand{\AnAction}  { {A}}
\newcommand{\anaction}  { {a}}
\newcommand{\ActionSpace}       { {\mathbf{\AnAction}}}

% Abbreviations from RURO:
\newcommand{\InfoGain}[2] { \mathcal{D} \left( {#1} || {#2} \right) }

% Abbreviations from Upper Bound:
\newcommand{\lcm}       {{\rm lcm}}
% Double-check that this isn't in the math set already!

% Abbreviations from Emergence in Space
\newcommand{\ProcessAlphabet}   {\MeasAlphabet}
\newcommand{\ProbEst}                   { {\widehat{\Prob}_N}}
\newcommand{\STRegion}                  { {\mathrm K}}
\newcommand{\STRegionVariable}          { K}
\newcommand{\stregionvariable}          { k}
\newcommand{\GlobalPast}                { \overleftarrow{G}}
\newcommand{\globalpast}                { \overleftarrow{g}}
\newcommand{\GlobalFuture}              { \overrightarrow{G}}
\newcommand{\globalfuture}              { \overrightarrow{g}}
\newcommand{\GlobalState}               { \mathcal{G}}
\newcommand{\globalstate}               { \gamma}
\newcommand{\GlobalStateSet}            { {\mathbf \GlobalState}}
\newcommand{\LocalPast}                 { \overleftarrow{L}}
\newcommand{\localpast}                 { \overleftarrow{l}}
\newcommand{\AllLocalPasts}             { \mathbf{\LocalPast}}
\newcommand{\LocalPastRegion}           { \overleftarrow{\mathrm L}}
\newcommand{\LocalFuture}               { \overrightarrow{L}}
\newcommand{\localfuture}               { \overrightarrow{l}}
\newcommand{\LocalFutureRegion}         { \overrightarrow{\mathrm L}}
\newcommand{\LocalState}                { \mathcal{L}}
\newcommand{\localstate}                { \lambda}
\newcommand{\LocalStateSet}             { {\mathbf \LocalState}}
\newcommand{\PatchPast}                 { \overleftarrow{P}}
\newcommand{\patchpast}                 { \overleftarrow{p}}
\newcommand{\PatchPastRegion}           { \overleftarrow{\mathrm P}}
\newcommand{\PatchFuture}               { \overrightarrow{P}}
\newcommand{\patchfuture}               { \overrightarrow{p}}
\newcommand{\PatchFutureRegion}         { \overrightarrow{\mathrm P}}
\newcommand{\PatchState}                { \mathcal{P}}
\newcommand{\patchstate}                { \pi}
\newcommand{\PatchStateSet}             { {\mathbf \PatchState}}
\newcommand{\LocalStatesInPatch}        {\vec{\LocalState}}
\newcommand{\localstatesinpatch}        {\vec{\localstate}}
\newcommand{\PointInstantX}             { {\mathbf x}}
% Galles's original LaTeX for the cond. indep. symbol follows:
\newcommand{\compos}{\mbox{$~\underline{~\parallel~}~$}}
\newcommand{\ncompos}{\not\hspace{-.15in}\compos}
\newcommand{\indep}                     { \rotatebox{90}{$\models$}}
\newcommand{\nindep}    {\not\hspace{-.05in}\indep}
\newcommand{\LocalEE}   {{\EE}^{loc}}
\newcommand{\EEDensity} {\overline{\LocalEE}}
\newcommand{\LocalCmu}  {{\Cmu}^{loc}}
\newcommand{\CmuDensity}        {\overline{\LocalCmu}}

%%%%%%%%%%% added by sasa
\newcommand{\FinPast}[1]        { \overleftarrow {\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finpast}[1]        { \overleftarrow {\meassymbol}  \stackrel{{#1}}{}}
\newcommand{\FinFuture}[1]              { \overrightarrow{\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finfuture}[1]              { \overrightarrow{\meassymbol} \stackrel{{#1}}{}}

\newcommand{\Partition} { \AlternateState }
\newcommand{\partitionstate}    { \alternatestate }
\newcommand{\PartitionSet}      { \AlternateStateSet }
\newcommand{\Fdet}   { F_{\rm det} }

\newcommand{\Dkl}[2] { D_{\rm KL} \left( {#1} || {#2} \right) }

\newcommand{\Period}    {p}

% To take into account time direction
\newcommand{\forward}{+}
\newcommand{\reverse}{-}
%\newcommand{\forwardreverse}{\:\!\diamond} % \pm
\newcommand{\forwardreverse}{\pm} % \pm
\newcommand{\FutureProcess}     { {\Process}^{\forward} }
\newcommand{\PastProcess}       { {\Process}^{\reverse} }
\newcommand{\FutureCausalState} { {\CausalState}^{\forward} }
\newcommand{\futurecausalstate} { \sigma^{\forward} }
\newcommand{\altfuturecausalstate}      { \sigma^{\forward\prime} }
\newcommand{\PastCausalState}   { {\CausalState}^{\reverse} }
\newcommand{\pastcausalstate}   { \sigma^{\reverse} }
\newcommand{\BiCausalState}             { {\CausalState}^{\forwardreverse} }
\newcommand{\bicausalstate}             { {\sigma}^{\forwardreverse} }
\newcommand{\FutureCausalStateSet}      { {\CausalStateSet}^{\forward} }
\newcommand{\PastCausalStateSet}        { {\CausalStateSet}^{\reverse} }
\newcommand{\BiCausalStateSet}  { {\CausalStateSet}^{\forwardreverse} }
\newcommand{\eMachine}  { M }
\newcommand{\FutureEM}  { {\eMachine}^{\forward} }
\newcommand{\PastEM}    { {\eMachine}^{\reverse} }
\newcommand{\BiEM}              { {\eMachine}^{\forwardreverse} }
\newcommand{\BiEquiv}   { {\sim}^{\forwardreverse} }
\newcommand{\Futurehmu} { h_\mu^{\forward} }
\newcommand{\Pasthmu}   { h_\mu^{\reverse} }
\newcommand{\FutureCmu} { C_\mu^{\forward} }
\newcommand{\PastCmu}   { C_\mu^{\reverse} }
\newcommand{\BiCmu}             { C_\mu^{\forwardreverse} }
\newcommand{\FutureEps} { \epsilon^{\forward} }
\newcommand{\PastEps}   { \epsilon^{\reverse} }
\newcommand{\BiEps}     { \epsilon^{\forwardreverse} }
\newcommand{\FutureSim} { \sim^{\forward} }
\newcommand{\PastSim}   { \sim^{\reverse} }
\newcommand{\FuturePC}  {\PC^{\forward}}
\newcommand{\PastPC}            {\PC^{\reverse}}
\newcommand{\BiPC}      {\PC^{\forwardreverse}}

% Used arrows for awhile, more or less confusing?
%\newcommand{\FutureCausalState}        { \overrightarrow{\CausalState} }
%\newcommand{\PastCausalState}  { \overleftarrow{\CausalState} }
%\newcommand{\eMachine} { M }
%\newcommand{\FutureEM} { \overrightarrow{\eMachine} }
%\newcommand{\PastEM}   { \overleftarrow{\eMachine} }
%\newcommand{\FutureCmu}        { \overrightarrow{\Cmu} }
%\newcommand{\PastCmu}  { \overleftarrow{\Cmu} }

%% time-reversing and mixed state presentation operators
\newcommand{\TR}{\mathcal{T}}
\newcommand{\MSP}{\mathcal{U}}
\newcommand{\one}{\mathbf{1}}

%% added for RURO2
%% Note that it will always be typesett in math mode.
%% Example usage:
%%    The 3-block entropy is \BE[t]{3}.
%%    The 3-block-state entropy from $t=0$ is $\BSE{3}$.
%%
%% The optional argument specifies the start time, defaulting to t=0.
%% The mandatory argument specifies the length of the block (not the stop time).
\newcommand{\lastindex}[2]{
  \edef\tempa{0}
  \edef\tempb{#2}
  \ifx\tempa\tempb
    % if the length is 0, then the final time equals the start time
    \edef\tempc{#1}
  \else
    % if the start time is different from zero, then we show the sum
    \edef\tempa{0}
    \edef\tempb{#1}
    \ifx\tempa\tempb
      \edef\tempc{#2}
    \else
      \edef\tempc{#1+#2}
    \fi
  \fi
  \tempc
}
\newcommand{\BE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\BSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\CausalState_{\lastindex{#1}{#2}}]}%
}
\newcommand{\SBE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\SBSE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2},
                \CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\AltBSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBSE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2},
                \AlternateState_{\lastindex{#1}{#2}}]}
}

\newcommand{\GI}{\ensuremath{\varphi}\xspace}
\newcommand{\OI}{\ensuremath{\zeta}\xspace}
% cryptic, gauge, oracular, Markov, and synchronization
\newcommand{\COrder}{\ensuremath{k_{\PC}}\xspace}
\newcommand{\GOrder}{\ensuremath{k_{\GI}}\xspace}
\newcommand{\OOrder}{\ensuremath{k_{\OI}}\xspace}
\newcommand{\MOrder}{\ensuremath{R}\xspace}
\newcommand{\SOrder}{\ensuremath{k_{\SI}}\xspace}


%% Added to standardize the order of causal states
%% Example usage:
%%    $\BiCmu = H[\CSjoint] = H[\CSjoint[,]]$
%%    $\EE = I[\CSjoint[:]] = I[\CSjoint[;]]$
\newcommand{\CSjoint}[1][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState\!#1\PastCausalState}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState#1\PastCausalState}
   \fi
}
\newcommand{\CSjointKL}[3][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState_{#2}\!#1\PastCausalState_{#3}}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState_{#2}#1\PastCausalState_{#3}}
   \fi
}


%% (cje)
%% Provide a command \ifpm which is true when \pm
%% is meant to be understood as "+ or -", opposed
%% to "bidirectional". This differs from the usage
%% in TBA.  Essentially, if \forwardreverse is defined
%% as something different, perhaps a \diamond, then
%% we are free to interpret \pm as "+ or -".
\newif\ifpm
\edef\tempa{\forwardreverse}
\edef\tempb{\pm}
\ifx\tempa\tempb
   \pmfalse
\else
   \pmtrue
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metric quantities of information generation, eg anatomy of a bit

\newcommand{\metric}[1] {\ensuremath{#1_\mu}\xspace}

\renewcommand{\hmu}{\metric{h}}
\newcommand{\rhomu}{\metric{\rho}}
\newcommand{\rmu}{\metric{r}}
\newcommand{\bmu}{\metric{b}}
\newcommand{\qmu}{\metric{q}}
\newcommand{\wmu}{\metric{w}}
\newcommand{\imu}{\metric{i}}
\newcommand{\sigmamu}{\metric{\sigma}}

\newcommand{\himc}{\ensuremath{h_{imc}}\xspace}
\newcommand{\pee}{\ensuremath{pee}\xspace} % parallel edge entropy

\newcommand{\ExE}[1] {\ensuremath{\EE_{#1}}\xspace}

\newcommand{\EER}{\ExE{R}}
\newcommand{\EEB}{\ExE{B}}
\newcommand{\EEQ}{\ExE{Q}}
\newcommand{\EEW}{\ExE{W}}
\newcommand{\EI}{\mathbf{I}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time series, using the python-esque notation

\newcommand{\MS} [2] {\ensuremath{\MeasSymbol_{#1:#2}}\xspace}
\newcommand{\ms} [2] {\ensuremath{\meassymbol_{#1:#2}}\xspace}

\renewcommand{\Past}       {\MS{}{0}}
\newcommand{\Present}      {\ensuremath{\MeasSymbol_{0}}\xspace}
\renewcommand{\Future}     {\MS{0}{}}
\newcommand{\LPresent} [1] {\MS{0}{#1}}
\newcommand{\LFuture}  [1] {\MS{#1}{}}

\renewcommand{\past}       {\ms{}{0}}
\newcommand{\present}      {\ensuremath{\meassymbol_{0}}\xspace}
\renewcommand{\future}     {\ms{0}{}}
\newcommand{\lpresent} [1] {\ms{0}{#1}}
\newcommand{\lfuture}  [1] {\ms{#1}{}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Causal states

\newcommand{\FCS}{\CausalState^\forward\xspace}
\newcommand{\RCS}{\CausalState^\reverse\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Others

\newcommand{\half}{\ensuremath{\nicefrac{1}{2}}}

\newcommand{\Language} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Lsync} {\Language_{\mathrm{sync}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathclap, in case someone doesn't have mathtools

% TUGboat, Volume 0 (2001), No. 0
% http://math.arizona.edu/~aprl/publications/mathclap/perlis_mathclap_24Jun2003.pdf
% For comparison, here are the existing overlap macros:
% \def\llap#1{\hbox to 0pt{\hss#1}}
% \def\rlap#1{\hbox to 0pt{#1\hss}}
%
% These are provided by mathtools
%
\ifcsname mathclap\endcsname
  \relax
\else
  \def\clap#1{\hbox to 0pt{\hss#1\hss}}
  \def\mathllap{\mathpalette\mathllapinternal}
  \def\mathrlap{\mathpalette\mathrlapinternal}
  \def\mathclap{\mathpalette\mathclapinternal}
  \def\mathllapinternal#1#2{%
    \llap{$\mathsurround=0pt#1{#2}$}}
  \def\mathrlapinternal#1#2{%
    \rlap{$\mathsurround=0pt#1{#2}$}}
  \def\mathclapinternal#1#2{%
    \clap{$\mathsurround=0pt#1{#2}$}}
\fi


==> infotheory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Information theory macros

\def \mid {~\middle|~}

% functions
\newcommand{\op}  [2]   {\ensuremath{\operatorname{#1}\left[#2\right]}\xspace}

% entropies
\renewcommand{\H}  [1]          {\op{H}{#1}}
\newcommand{\ReE}  [2] [\alpha] {\op{H_{#1}}{#2}}
\newcommand{\TsE}  [2] [q]      {\op{S_{#1}}{#2}}
\newcommand{\CRE}  [1]          {\op{\mathcal{E}}{#1}}
\newcommand{\GCRE} [1]          {\op{\mathcal{E^\prime}}{#1}}

% mutual informations
\newcommand{\I}  [1] {\op{I}{#1}}
\newcommand{\T}  [1] {\op{T}{#1}}
\newcommand{\B}  [1] {\op{B}{#1}}
\newcommand{\J}  [1] {\op{J}{#1}}
\newcommand{\II} [1] {\op{II}{#1}}

% common informations
\newcommand{\K} [1] {\op{K}{#1}}
\newcommand{\C} [1] {\op{C}{#1}}
\newcommand{\G} [1] {\op{G}{#1}}
\newcommand{\F} [1] {\op{F}{#1}}
\newcommand{\M} [1] {\op{M}{#1}}

% transfer entropies
\newcommand{\TE} [2] {\ensuremath{\operatorname{T}_{#1\rightarrow#2}}\xspace}
\newcommand{\CE} [3] {\ensuremath{\operatorname{\mathcal{C}}_{#1\rightarrow#2|#3}}\xspace}

% others
\renewcommand{\P}    [1] {\op{P}{#1}}
\newcommand{\X}    [1] {\op{X}{#1}}
\newcommand{\R}    [1] {\op{R}{#1}}
\newcommand{\D}    [1] {\op{D}{#1}}
\newcommand{\LMRP} [1] {\op{C_{\textrm{LMRP}}}{#1}}
\newcommand{\TSE}  [1] {\op{TSE}{#1}}

% divergences
\newcommand{\divergence} [3] {\ensuremath{\operatorname{#1}\left[#2~\middle|\middle|~#3\right]}\xspace}

\newcommand{\xH}  [2] {\divergence{xH}{#1}{#2}}
\newcommand{\DKL} [2] {\divergence{D_{KL}}{#1}{#2}}
\newcommand{\JSD} [2] {\divergence{D_{JS}}{#1}{#2}}

% operators on random variables
\newcommand{\meet}      {\curlywedge}
\newcommand{\join}      {\curlyvee}
\newcommand{\iless}     {\preceq}
\newcommand{\imore}     {\succeq}
\newcommand{\ieq}       {\cong}
\newcommand{\mss}       {\searrow}

\newcommand{\ind}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}

\DeclareMathOperator*{\meetop}{\scalerel*{\meet}{\textstyle\sum}}
\DeclareMathOperator*{\joinop}{\scalerel*{\join}{\textstyle\sum}}

